Variance-Reduced Off-Policy Memory-Efficient Policy Search

Off-policy policy optimization is a challenging problem in reinforcement learning (RL). The algorithms designed for this problem often suffer from high variance in their estimators, which results in poor sample efficiency, and have issues with convergence. A few variance-reduced on-policy policy gradient algorithms have been recently proposed that use methods from stochastic optimization to reduce the variance of the gradient estimate in the REINFORCE algorithm. However, these algorithms are not designed for the off-policy setting and are memory-inefficient, since they need to collect and store a large ``reference'' batch of samples from time to time. To achieve variance-reduced off-policy-stable policy optimization, we propose an algorithm family that is memory-efficient, stochastically variance-reduced, and capable of learning from off-policy samples. Empirical studies validate the effectiveness of the proposed approaches.

==> Variance-Reduced Off-Policy Memory-Efficient Policy Search/exp.tex <==
\section{Experiments and Results}
\label{sec:exp}
The experiments are conducted to investigate the following questions empirically. i) How do VOMPS\&ACE-STORM compare with state-of-art off-policy policy gradient methods, such as GeoffPAC~\citep{geoffpac}, ACE, DDPG~\citep{lillicrap2015continuous}, and TD3~\citep{fujimoto2018addressing}?  ii) How do VOMPS\&ACE-STORM compare with on-policy variance-reduced policy gradient methods, e.g., SVRPG~\citep{svrpg} and SRVR-PG~\citep{sarahpg}? iii) How is VOMPS\&ACE-STORM resilient to action noise in policy gradient methods?

Since the tasks for original domains are episodic, e.g., \texttt{CartPoleContinuous-v0}, \texttt{Hopper-v2} and \texttt{HalfCheetah-v2}, we modify them as continuing tasks following ~\citep{geoffpac}--- the discount factor $\gamma$ is set to $0.99$ for all non-terminal states and $0$ for terminal states. The environment is reset to the initial state if the agent reaches the terminal state.
Therefore, simulation-based cumulative rewards (Monte Carlo return) by executing the (learned) policy $\pi$ is used as the performance metric, while results of episodic return are also provided in the Appendix.
All the curves in the results are averaged over $10$ runs, where the solid curve indicates the mean and the shaded regions around the mean curve indicate standard deviation errors. To better visualize the plots, curves are smoothed by a window of size
$20$. Shorthands ``1K'' represents $10^3$, and ``1M'' represents $10^6$. 
In the off-policy setting, the behavior policy $\mu$ follows a fixed uniform distribution. VOMPS, ACE-STORM, GeoffPAC, and ACE have the same critic component in all experiments for a fair comparison.
%


\subsection{Tabular off-policy policy gradient}
%
We first compare the performance of ACE, GeoffPAC, ACE-STORM, and VOMPS on the two-circle MDP domain~\citep{imani2018off,geoffpac} in terms of their dynamic and asymptotic solutions. In the two-circle MDP, there are a finite number of states, and an agent only decides at state \texttt{A} on either transitioning to state \texttt{B} or state \texttt{C}, whereas the transitions at other states will always be deterministic. The discount factor $\gamma = 0.6$ and rewards are $0$ unless specified on the edge as shown in Fig.~\ref{fig:circle}.
%
\begin{figure*}[htb!]
\begin{subfigure}{.5\textwidth}
  \centering
%   \includegraphics[height=3.5cm,width=4cm]{figures/two-circle.png}
    \includegraphics[height=2.5cm,width=.6\textwidth]{figures/two-circle.png}
  \caption{Two-circle MDP}
  \label{fig:circle}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
%   \includegraphics[height=5.0cm,width=7cm]{figures/CircleMDP_prob.png}
    \includegraphics[height=3.0cm,width=.8\textwidth]{figures/CircleMDP_prob.png}
  \caption{The probability of transitioning from A to B}
  \label{fig:circle_result}
\end{subfigure}
\caption{The two-circle MDP}
\end{figure*}
%
The algorithms for this domain, GeoffPAC, ACE, VOMPS, and ACE-STORM, are implemented with a tabular version, where value function and density ratio function is computed via dynamic programming. The behavior policy $\mu$ follows a uniform distribution, and $\pi(A \rightarrow B)$, the probability from A to B under the target policy $\pi$ is reported in  Fig.~\ref{fig:circle_result}. 
As shown in Fig.~\ref{fig:circle_result}, VOMPS and GeoffPAC gradually choose to transition from A to B so that the agent would take the route with blue color and obtain a reward of $+10$. Compared with GeoffPAC, VOMPS converges faster.
Both ACE-STORM and ACE move from A to C, and ACE-STORM converges faster than ACE. Moving from A to C is an inferior solution since the agent will take the route with green color and fail to obtain a higher reward.
The difference between asymptotic solutions of GeoffPAC/VOMPS and ACE/ACE-STORM is due to the difference between the objective functions $J_{\hat \gamma}, J_\mu$, and the difference in the training process is due to the STORM component integrated into VOMPS and ACE-STORM.

\begin{figure*}[htb!]
\centering
\begin{subfigure}{.44\textwidth}
  \centering
  \includegraphics[height=3.5cm,width=1.\textwidth]{figures/cartpole_smooth_onpol.png}
  \caption{Comparison with on-policy methods}
  \label{fig:cartpole:onpol}
\end{subfigure}
\begin{subfigure}{.44\textwidth}
  \centering
  \includegraphics[height=3.5cm,width=1.\textwidth]{figures/cartpole_smooth_offpol.png}
  \caption{Comparison with off-policy methods}
  \label{fig:cartpole:offpol}
\end{subfigure}
\caption{Results on \texttt{CartPoleContinuous-v0}}
\end{figure*}

\subsection{Classic Control}
We use \texttt{CartPoleContinuous-v0} for CartPole domain, which has a continuous action space within the range of $[-1,1]$.
A near-optimal policy can reach a Monte-Carlo return at the level of $57$ within a fixed horizon of $200$ timesteps.
As shown in Fig.~\ref{fig:cartpole:onpol}, VOMPS and ACE-STORM learn the near-optimal policy with around $200$K samples, while SVRPG and SRVR-PG need more than $400$K samples with larger dynamic variances. As Fig.~\ref{fig:cartpole:offpol} shows, ACE, GeoffPAC, and DDPG do not perform well in this domain. Although TD3 seems to learn faster at the beginning, it reaches an inferior solution with a mean return around $50$ a higher variance than VOMPS and ACE-STORM.


\subsection{Mujoco Robot Simulation}
Experiments are also conducted on two benchmark domains provided by OpenAI Gym, including \texttt{Hopper-v2} and \texttt{HalfCheetah-v2}. 
As shown in Fig.~\ref{fig:hopper:onpol},~\ref{fig:hopper}, both GeoffPAC and VOMPS can achieve higher Monte Carlo returns than other methods and converge faster within $1$M samples on \texttt{Hopper-v2}. Compared with GeoffPAC, the learning curve of VOMPS is smoother and has a smaller variance. 
The results on \texttt{HalfCheetah-v2} are shown in Fig.~\ref{fig:halfcheetah:onpol},~\ref{fig:halfcheetah}. Fig.~\ref{fig:halfcheetah:onpol} indicates that VOMPS and ACE-STORM outperform SVRPG and SRVR-PG by a large margin, and Fig.~\ref{fig:halfcheetah} demonstrates that VOMPS and ACE-STORM achieve a similar performance of GeoffPAC/DDPG/TD3, with obviously smaller variances. We also observe that ACE does not perform well in general, and DDPG has a very large variance in these two domains.

In addition, a $20\%$ action noise is added to both the learning process and evaluation process in order to compare the noise resistance ability of different approaches (aka, the action is multiplied by a factor of $1\pm 0.2\chi$, where $\chi$ is drawn from a $[0,1]$-range uniform distribution). As shown in Fig.~\ref{fig:hopper:noise:onpol},~\ref{fig:hopper:noise:offpol},~\ref{fig:halfcheetah:noise:onpol},~\ref{fig:halfcheetah:noise:offpol}, compared with results under the original noise-free setting, VOMPS, ACE-STORM, SVRPG, and SRVR-PG tend to be insensitive to disturbances than other methods, which validates the effectiveness of the stochastic variance reduction component of these algorithms. In particular, VOMPS and ACE-STORM appear to be empirically the most noise-resistant in these two domains. 



\begin{footnotesize}
\begin{figure*}[htb!]
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width = 1\textwidth]{figures/hopper_onp.png}
  \caption{Hopper}
  \label{fig:hopper:onpol}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width = 1\textwidth]{figures/halfcheetah_onpol.png}
    \caption{HalfCheetah}
    \label{fig:halfcheetah:onpol}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width = 1\textwidth]{figures/hop_20act_onpol.png}
  \caption{Hopper (action noise)}
  \label{fig:hopper:noise:onpol}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width = 1\textwidth]{figures/hc_20act_onpol.png}
  \caption{{\footnotesize HC (action noise)}}
  \label{fig:halfcheetah:noise:onpol}
\end{subfigure}
\caption{Comparison with on-policy PG methods (Mujoco), ``HC'' is short for HalfCheetah.}
\end{figure*}

\begin{figure*}[htb!]
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width = 1\textwidth]{figures/hopper_offp.png}
  \caption{Hopper}
  \label{fig:hopper}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width = 1\textwidth]{figures/halfcheetah_offpol.png}
    \caption{HalfCheetah}
    \label{fig:halfcheetah}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width = 1\textwidth]{figures/hop_20act_offpol.png}
  \caption{Hopper (action noise)}
  \label{fig:hopper:noise:offpol}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width = 1\textwidth]{figures/hc_20act_offpol.png}
    \caption{{\footnotesize HC (action noise)}}
  \label{fig:halfcheetah:noise:offpol}
\end{subfigure}
\caption{Comparison with off-policy PG methods (Mujoco), ``HC'' is short for HalfCheetah.}
\end{figure*}
\end{footnotesize}

==> Variance-Reduced Off-Policy Memory-Efficient Policy Search/theory.tex <==
\subsection{Theoretical Analysis}
%
In this section, we present a theoretical analysis of the VOMPS algorithm. To start, we first present the assumptions used in the study.
\begin{assumption}[\textbf{Bounded Gradient}]
\label{assump:grad}
\citep{svrpg,sarahpg}
Let $\pi_{\theta}(a|s)$ be the agent's policy at state $s$. There exist constants $W,U>0$ such that the log-density of the policy function satisfies:
% \begin{align}
$
\|\nabla_{\theta}\log \pi_{\theta}(a|s)\|_2\leq W,\quad \big\|\nabla_{\theta}^2\log \pi_{\theta}(a|s)\big\|_2\leq U,
$
% \end{align}
for $\forall$ $a\in\mathcal{A}$ and $s\in\mathcal{S}$, and $||\cdot||_2$ is the $\ell_2$ norm.
\end{assumption}

\begin{assumption}[\textbf{Lipschitz continuity and Bounded Variance}]\citep{xu2019improved,sarahpg,storm}
The estimation of policy gradient $Z(\theta)$ is bounded, Lipschitz continuous, and has a bounded variance, i.e.,  
there exist constants $L, G, \sigma$ such that
$
\|Z(\theta_1) - Z(\theta_2)\|_2 \leq L\|\theta_1-\theta_2\|_2
$
for $\forall$ $\theta_1,\theta_2\in \mathbb{R}^d$, and $\|Z(\theta)\|_2 \leq G, \mathbb{E}[\|Z(\theta) -\nabla J_{\hat{\gamma}}(\theta)\|_2^2] \leq {\sigma}^2$ for $\forall$ $\theta\in\mathbb{R}^d$.
\end{assumption}

We now present our main theoretical result, the convergence analysis of Algorithm~\ref{alg:vomps}.
\begin{theorem}
Under the above assumptions, for any $b>0$, let $k=\frac{b \sigma^\frac{2}{3}}{L}$, $\beta=28L^2 + \sigma^2/(7 L k^3) = L^2(28 + 1/(7 b^3))$, and $w=\max\left((4Lk)^3, 2\sigma^2, \left(\tfrac{\beta k}{4 L}\right)^3\right) = \sigma^2\max\left((4 b)^3, 2, (28b+\frac{1}{7b^2})^3/64\right)$. Then, the output of Algorithm~\ref{alg:vomps} satisfies
\begin{align}
    \mathbb{E} \left[\|\nabla J_{\hat{\gamma}}(\hat{\theta})\|^2\right]
= \mathbb{E} \left[\frac{1}{T}\sum_{t=1}^T \|\nabla J_{\hat{\gamma}}(\theta_t)\|^2\right]
\leq \frac{40\Delta_{\Phi}}{T^{2/3}} + \frac{2\beta^2\sigma^2}{L^2T^{2/3}},
\end{align}
where $\Delta_{\Phi} \leq \Delta_{J_{\hat{\gamma}}} + \frac{\|\epsilon_0\|^2}{32\eta_0L^2},\Delta_{J_{\hat{\gamma}}} =   J_{\hat{\gamma}}(\theta^*)-J_{\hat{\gamma}}(\theta) , \forall \theta\in R^d$, and $\theta^\star$ is the maximizer of $J_{\hat{\gamma}}$.
\label{thm:vomps}
\end{theorem}
Theorem~\ref{thm:vomps} indicates that VOMPS requires $O(1/\epsilon^{3/2})$ samples to find an $\epsilon$-stationary point. As VOMPS is developed based on GeoffPAC and STORM, the proof of convergence rates of VOMPS is similar to STORM. 
 However, the proof is not a trivial extension by merely instantiating the objective function to $J_{\hat{\gamma}}$ in the RL settings.
  If we just apply the original analysis of STORM, we can only achieve $O(\frac{\log(1/\epsilon)}{\epsilon^{2/3}})$. 
In \cite{ yuan2020stochastic}, it improves the sample complexity to $O(1/\epsilon^{2/3})$ by introducing the large mini-batch $O(1/\sqrt{\epsilon})$ and using extremely small stepsize $o(\epsilon)$. 
Nevertheless the improved sample complexity, 
the introduced $O(1/\sqrt{\epsilon})$ mini-batch size will lead to memory inefficiency, and the $O(\epsilon)$ stepsize will slow down the training process. VOMPS overcomes the above two weaknesses and achieves the $O(1/\epsilon^{2/3})$ sample complexity by applying increasing weights strategy and an automatically adjusted stepsize strategy that proportions to iterations. These techniques are not used in the original STORM method. As a result, VOMPS is the first variance reduced memory-efficient off-policy method that achieves the optimal sample complexity, which matches the lower-bound provided in~\cite{arjevani2019lower}.

\begin{table}[ht]%{r}{0.5\linewidth}
 %\vspace{-0.1in}
 \begin{center}
 \begin{tabular}{c c c c c}
 \toprule
 {Algorithms}   & Objective & {Sample Complexity}  & {Off-Policy?} 
  & {Required Batch} \\ 
 \toprule
 SVRPG \citep{svrpg}  & $J_\pi$ &$O(1/{\epsilon ^2})$ &$\times$   & $O(1/{\epsilon})$ \\
 SVRPG \citep{xu2019improved} & $J_\pi$ &$O(1/{\epsilon ^{5/3}})$ &$\times$ 
  & $O(1/{\epsilon^{2/3}})$ \\
 SRVR-PG \citep{sarahpg} & $J_\pi$ & $O(1/{\epsilon ^{3/2}})$ &$\times$ 
  & $O(1/{\epsilon^{1/2}})$ \\
 ACE-STORM (This paper)  & $J_{\mu}$ & $O(1/{\epsilon ^{3/2}})$ & \checkmark   & $\times$ \\
 VOMPS (This paper) & $J_{\hat \gamma}$ & $O(1/{\epsilon ^{3/2}})$ & \checkmark   & $\times$\\
 \bottomrule
 \end{tabular}
 \end{center}
 %\vspace{-0.15in}
 \begin{footnotesize}
 \caption{\label{table:pg_rate}{\footnotesize Comparison on convergence rate of different algorithms when $\|\nabla J(\theta)\|_2^2 \leq \epsilon$. The $\times$ in ``Required Batch'' means that no mini-batch is needed, aka, the algorithm is memory efficient.}}
 \end{footnotesize}
 \end{table}
\begin{remark}
Theorem~\ref{thm:vomps} indicates that VOMPS enjoys the same convergence rate as the state-of-the-art algorithms together with SRVR-PG~\citep{sarahpg}. A summary of state-of-the-art convergence rate is summarized in Table~\ref{table:pg_rate}.
It should be noted that unlike other algorithms that optimize $J_\pi$, the objective function of VOMPS is $J_{\hat \gamma}$. However, these two objective functions only differ in constants in the on-policy setting. Thus, it is a fair comparison of the convergence rate. 
\end{remark}


\subsection{ACE-STORM Algorithm Design}
As an extension, we also propose the \textbf{A}ctor-\textbf{C}ritic with \textbf{E}mphatic weighting and \textbf{STO}chastic \textbf{R}ecursive \textbf{M}omentum (ACE-STORM) algorithm, which is an integration of the ACE algorithm~\citep{imani2018off} and STORM~\citep{storm}. Similar to discussed above, the objective of ACE-STORM is also a special case of that in Algorithm~\ref{alg:vomps} by setting $\hat \gamma = 0$. The pseudo-code of the ACE-STORM Algorithm is presented in the Appendix due to space constraints.




